Improving Continual Relation Extraction through Prototypical Contrastive Learning

Continual relation extraction (CRE) aims to extract relations towards the continuous and iterative arrival of new data, of which the major challenge is the catastrophic forgetting of old tasks. In order to alleviate this critical problem for enhanced CRE performance, we propose a novel Continual Relation Extraction framework with Contrastive Learning, namely CRECL, which is built with a classification network and a prototypical contrastive network to achieve the incremental-class learning of CRE. Specifically, in the contrastive network a given instance is contrasted with the prototype of each candidate relations stored in the memory module. Such contrastive learning scheme ensures the data distributions of all tasks more distinguishable, so as to alleviate the catastrophic forgetting further. Our experiment results not only demonstrate our CRECL's advantage over the state-of-the-art baselines on two public datasets, but also verify the effectiveness of CRECL's contrastive learning on improving CRE performance.

==> method-bak.tex <==
\section{Methodology}
 In this section, we introduce our CRE framework in detail. At first, we formalize the task of CRE addressed in this paper, and then overview our framework, followed by the detailed introduction of each component (step) of the framework.%在本节中，我们详细的阐述了我们的CRE框架。首先我们公式化了CRE问题和我们所使用的记忆模块。然后我们介绍了我们的模型结构，其主要由两个部分组成，如图，左半部分是对当前任务的分类网络，右半部分是对比网络。为了让我们的整体流程更容易理解，我们在介绍网络结构的同时会对由这两个网络引出的训练方法加以介绍。

% 为了方便描述，图中虚线框对应结构被称为encoder layer。左半边中句子中通过BERT后，其句子的实体特殊标识符$[E11]$,$[E12]$,$[E21]$,$[E22]$拼接后形成句子的表示向量。而所有instance在Hidden和Classifier Layer会进行$m$次前向传播，并由交叉熵保证这m个结果的正确性，由JSD保证m个结果的一致性。右图中训练实例和由memory中存储的实例经过encoder layer平均化后得到的原型进行对比学习训练。右图中对比网络虚线框与左图分类网络虚线框的encoder的参数共享。对比网络的实线框encoder参数不参与后向传播，固定为对比学习开始前的值。

\subsection{Task Formalization}
The CRE task aims to identify the relation between two entities expressed by one sentence in the task sequence. Formally, given a sequence of $K$ tasks $\{T_1,T_2,\ldots,T_K\}$, where the $k$-th task $T_k$ has its own samples $D_k$ and relation class set (relational schema) $\mathcal{R}_k$. $D_k$ contains $N_k$ instances $\{(x_1,t_1,y_1),\ldots,(x_{N_k},t_{N_k},y_{N_k})\}$ where instance $(x_i,t_i,y_i),1\leq i\leq N_k$ indicates that the relation of entity pair $t_i$ in sentence $x_i$ is $y_i \in \mathcal{R}_k$. 
% There are no identical relations in the $R_k$. 
One CRE model should perform well not only for the relations in $\mathcal{R}_k$ but also for the relations on all historical tasks up to $T_k$, denoted as $\tilde{\mathcal{R}}_k =\cup_{i=1}^k \mathcal{R}_i$. We also adopt an episodic memory module $\mathcal{M}_r = \{(x_1,t_1,r),\ldots,(x_L,t_L,r)\}$ to store typical instances of relations $r$, similar to \cite{wu2019enriching,han2020continual,cui2021refining}, where $L$ is the memory size (typical instance number). The overall episodic memory for the observed relations in all historical tasks up to now is $\tilde{\mathcal{M}}_k= \cup_{r \in \tilde{\mathcal{R}}_k} \mathcal{M}_r$. 
%每个任务有不重复的Rk，CRE模型需要不仅仅在Tk任务而且在当前所有T_K~=bingT_k上表现良好。也就是说模型需要应对一个逐渐增加的关系类别集合R~k=。memory如何如何。

Previous studies \cite{cui2021refining} assume the whole relation set $\tilde{\mathcal{R}}_k$ in all tasks is known at the beginning. However, in real scenarios, as the relations gradually come as each task arrives, the relation set $\mathcal{R}_k$ in current task $T_k$ is known only when $T_k$ arrives.
%以往的研究中\cite{cui2021refining}假设了一开始就已经知道全集的R~K集合，但实际中由于关系是每个任务逐渐到来的，因此当任务到来的时候,才应该知道其关系集合Rk.(K是总计的任务集合和关系集合k是当前关系集合。）

\subsection{Framework Overview} 
At first, we overview the architecture of our proposed CRE framework, which is shown in Figure \ref{fig:framework}. As formalized in  Algorithm \ref{alg1}, the operations in our framework can be mainly divided into two parts.
% 在本节中我们详细阐述了我们的框架整体的运行流程。正如图片\ref{fig:framework}、算法\ref{alg1}所示，我们的框架从结构上主要分为两个部分，从训练上来说会进行三次训练。

%The left part is a relation classification network that uses special tokens to strengthen entities and uses regularized dropout to obtain an accurate encoder and prototype in this task. 
The left part is a relation classification network that is fed with the instance representations in current task, and adopts regularized dropout to train an accurate encoder subjected to the real labels (relation class) of instances. Then, with the instance representations generated by the encoder, we apply K-means algorithm to select $L$ typical instances to represent each relation in current task, which are used to generate the relation prototypes and stored into the memory module for the subsequent usage. It is worth noting that the classification network serves only for current task, so it is only necessary to set its layer parameters according to the relation number in current task instead of the relation number in all tasks. It saves a lot of parameter cost compared with previous CRE models.
%左半边是一个使用了特殊tokens来加强实体和使用了多次dropout作为正则化技术的分类网络，其有两个目的：1.将当前任务中每种数据较为清楚的分开。2.训练一个准确的编码层来得到本轮任务中每种关系的嵌入向量，然后使用kmeans算法为每个类来选择出L个有代表性的数据放入到我们的memory中。值得注意的是，分类网络只需要负责当前任务，因此只需要在分类时只需要将分类层参数设置为每个任务的关系数而不是全部任务的关系数目。

The right half is a contrastive network used for comparing instances with the prototypes of the stored relations in the memory module. The objective of this contrastive network is to adjust the data (instances) distributions of all tasks to be more distinguishable, which can alleviate the catastrophic forgetting in CRE as we claimed before. Therefore, it is necessary to serve for both current task and historical tasks, so there are two training processes with this network. The first is to compare between current task instances and the relation prototypes stored in the memory module, which is used to help the contrastive model quickly learn the difference between the instances in current task and all stored relation prototypes. The second is to compare each typical instance and the relation prototypes that are both stored in the memory module, in order to help the model recall the relation prototypes in all previous tasks. %It is worth noting that the encoder layer in the contrastive network and the encoder layer in the classification network are parameter sharing (the dotted box in Figure \ref{fig:framework}), while the parameter of the solid box in the contrastive learning is fixed as the value before the start of the contrastive training, which ensure that the generated prototypes are not disturbed by the training, and make the distribution more uniform through contrastive learning.
%右半边是一个基于原型和训练实例对比的对比学习网络，因为需要同时负责当前任务和历史任务，所以进行了两次训练，第一次是当前任务数据与原型进行的训练，旨在帮助对比学习模型快速学习到当前任务与原型的差异，第二次是memory中所存储数据与原型表示的对比训练，旨在帮助模型回顾之前任务从而减缓灾难性遗忘的发生。值得一提的是，对比学习网络中的encoder layer与分类网络中的encoder layer是参数共享的（图中虚线框），而对比学习中的实线框参数不参与更新，固定保持为对比训练开始前的值，这样做既可以保证生成的原型不会被对比学习训练所扰乱，也可以通过对比学习来调整使训练实例的嵌入的分布更为规整。

Next, we introduce the detailed operations in our CRE framework as follows.
%The following sections will give a detailed introduction to each part of our model in algorithmic flow order.
%接下来的几节会以算法流程顺序对我们模型的各个部分进行具体的介绍。

\subsection{Classification Network for Current Task}
Classification models have demonstrated good performance on the classification tasks of fixed classes, hence we take a classifier similar to the SOTA CRE model \cite{cui2021refining} as our classification network. We also use special tokens to represent the entities in instance sentences for better instance representation. In order to improve the effects of token embeddings, inspired by \cite{wu2021r}, we further adopt $M$ dropouts for regularization, and then add Jensen-Shannon divergence (JSD) \cite{majtey2005jensen} loss to ensure more consistent instance distribution for model performance gains.
% 分类模型已经证明在固定类别的任务中表现良好，每个任务已知的类别信息让应用这样良好效果的模型成为可能。左半边是我们的为得到当前任务的关系表示设计的分类模型。我们参考了崔立的模型结构，同样使用了对实体进行强调的特殊实体标识符。不同的是，为了进一步提升模型表征能力，我们参考R-dropout，设计了一种使用了m次dropout进行数据正则化，使用Jensen-Shannon divergence散度来保证输出分布尽量一致，使用交叉熵保证输出分布的正确性的方法，来提升模型性能的结构。
\subsubsection{Classification Network Operations}
Specifically, as shown in Figure \ref{fig:framework}, the head entity and tail entity in the instance sentence are represented by two special position tokens $[E11, E12]$ and $[E21, E22]$, respectively. The instance representation $\boldsymbol{e}\in\mathbb{R}^{2h}$ before the hidden layer is the concatenation of token embeddings of $[E11, E12]$ and $[E21, E22]$ generated by the BERT \cite{devlin2018bert} encoder, where $h$ is the dimension of two token embeddings. Then $\boldsymbol{e}$ is fed into the hidden layer to obtain the hidden embedding as
\begin{equation}\label{eq:dropout}
    \boldsymbol{h}=\operatorname{LN}\bigg(\operatorname{GELU}\big(\boldsymbol{W}\operatorname{Dropout}(\boldsymbol{e})+\boldsymbol{b}\big)\bigg)\in \mathbb{R}^{d},
\end{equation}
where $\boldsymbol{W} \in \mathbb{R}^{{d}\times {2h}}$ and $\boldsymbol{b}\in \mathbb{R}^d$ are both trainable parameters. $\operatorname{GELU}(\cdot)$ is the activation function \cite{hendrycks2016gaussian}, and $\operatorname{LN}(\cdot)$ is the operation of layer normalization \cite{ba2016layer}. In our framework, $\boldsymbol{h}$ is just regarded as the instance's representation.

Then, the probability distribution of instance $x$, denoted as $\mathcal{P}(x)$, is calculated based on $\boldsymbol{h}$ in the classifier layer as
\begin{equation}\label{eq:output}
    \mathcal{P}(x)=\operatorname{softmax}(\boldsymbol{W_1}\boldsymbol{h}+\boldsymbol{b_1}),
\end{equation}
where $\boldsymbol{W_1} \in \mathbb{R}^{R\times {d}}$ and $\boldsymbol{b_1} \in \mathbb{R}^{R}$ are trainable parameters. $R$ is the relation number of current task which is much less than of the relation number of all tasks.

\subsubsection{Storing Typical Instances for Relation Prototypes}\label{sec:proto}
As we mentioned before, for each relation in current task, we select some typical instances to represent it which are stored in the memory module for the subsequent comparisons. To this end, given a relation $r$, we first apply K-means algorithm upon the representations ($\boldsymbol{h}$) of all instances belonging to $r$, to cluster them into $L$ clusters. Then, for each cluster, we select the instance most closest to the centroid of this cluster as its typical instance. Thus, $L$ typical instances for relation $r$ are selected and then stored into the memory module. %Then use the encoder layer in the last step to get the embeddings. 

With the stored typical instances, we average their representations as the prototype (embedding) of relation $r$. Such prototype best represents $r$ since the $L$ typical instances have the minimal distance sum to the $L$ cluster centroids. 
%so it is contribution to our contrastive learning. Since the use of K-means is only to obtain an intermediate embedding, 
Another merit of such prototypes for representing relations is their insensitivity to the value of $L$. 
% 为了选择出一些能反映类别特征的典型样本，受之前工作启发，我们对分类模型计算出的向量h应用K-Means算法。我们对当前任务的每个类别的所有嵌入使用了K-means算法，然后选取出L个离L个质心最近的样本，放入memory之中。之后再使用第一步中的bert和middle层(之后统称为encoder层)得到L个向量的表示，然后对L个向量表示取均值得到我们最终的原型表示向量（图中实线框）。我们这么做的目的是希望得到一个中间向量表示，其到类间各个实例形成的向量的距离尽量的小，这会有利于对比学习进行调整参数。由于使用K-means的使用仅仅是为了获得向量的中间表示，所以我们的模型并不会对参数L非常敏感。


\subsubsection{Classification Network Training Objective}
In the classification network, we conduct $M$ times forward propagation in the hidden and the classifier layer as shown in Figure \ref{fig:framework}. Due to the randomness of dropout layer, we can get $M$ probability distributions for an instance $i$, denoted as $\mathcal{P}^m_i(1\leq m\leq M, 1\leq i\leq N_k)$. In order to make all instance distributions more consistent, we further consider the JSD loss for each instance $i$, calculated as
\begin{equation}\label{eq:jsd}
    \mathcal{L}_i^{J S D} =\sum_{m=1}^{M} D_{KL}\left(\mathcal{P}_{i}^{m} \| \mathcal{P}_i\right), 
\end{equation}
where $\mathcal{P}_i:=\sum_{m=1}^{M} \mathcal{P}_i^{m}$ and $D_{KL}(\cdot)$ is Kullback-Leibler (KL) divergence. 

Then, the overall learning objective of the classification network is the sum of $\mathcal{L}^{J S D}$ and the cross entropy loss $\mathcal{L}^{CE}$. Formally, the overall classification loss for current task $T_k$ is calculated as
%to minimize $\mathcal{L}^{i}_1$ for data ($x_i$,$y_i$) to regularize on the model predictions by applying the JSD and cross entropy between these $m$ output distributions $\mathcal{P}$ for the same sample
\begin{equation}\label{eq:enh}
\begin{aligned}
    \mathcal{L}_1=\mathcal{L}^{C E}+\alpha \mathcal{L}^{J S D} =\\
    -\frac{1}{N_k}\frac{1}{M}\bigg(\sum_{i=1}^{N_k} \sum_{m=1}^{M} \sum_{r=1}^{R} y_{i,r}^{m}\log \mathcal{P}_{i,r}^{m} &+\alpha \sum_{i=1}^{N_k}\sum_{m=1}^{M} D_{KL}\left(\mathcal{P}_{i}^{m} \| \mathcal{P}_{i}\right) \bigg)
\end{aligned}
\end{equation}
where $\alpha\in [0,1]$ is a controlling parameter and $y_{i,r}^{m}$ is instance $i$'s real relation label indicating whether $i$'s relation is relation $r$ (1 or 0). $\mathcal{P}_{i,r}^{m}$ is the $r$-th probability in the probability distribution $\mathcal{P}_{i}^{m}$ of instance $i$.
%After the above steps, a classification network with good performance for the current task is obtained.
%具体来说

%包含网络结构，loss公式。

% 通过以上步骤之后就得到了一个对当前任务性能良好的分类网络.
% 具体公式

\subsection{Contrastive Network for Refining Data Distributions}
In this contrastive network, we compare the instances and the relation prototypes (obtained through the stored typical instances) with supervised contrastive learning paradigm, to refine the data (instance) distributions of all tasks. As we illustrated in Section \ref{sec:classincre}, these refined data distributions help the model alleviate catastrophic forgetting. The basic principle of the comparisons is that, an instance's representation should be close to the prototype of its relation (positive sample), and be far away from the prototypes of the rest relations (negative samples). Please note that, the positive and negative samples in our contrastive learning are identified by the real labels of the training instances. Thus it is different to the self-supervised contrastive learning in other models \cite{chen2020simple}.

%Here we model contrastive learning as a comparison of a sentence with its prototype: the prototype itself is in the center of the class, and for those sentences that belong to the same class as the prototype, we think that it has similarities with the prototype, otherwise it should be treated as a negative sample. 

\subsubsection{Contrastive Learning Objective}
As shown in the right part of Figure \ref{fig:framework}, the contrastive network is built with a twin-tower architecture, where either tower mainly consists of the BERT encoder in the classification network and a projector. In the left tower, the representations of $L$ typical instances fetched from the memory module are first averaged as the relation prototype, namely $\boldsymbol{p}\in\mathbb{R}^{d}$, before being fed into the projector. Then, the compared embedding of the relation, namely $\mathbf{s}^r\in\mathbb{R}^{\frac{d}{2}}$, is obtained through the projector as
\begin{equation}\label{eq:project}
\begin{aligned}
    \mathbf{s}^r=\boldsymbol{W_3} \operatorname{GELU}(\boldsymbol{W_2}\boldsymbol{p}+\boldsymbol{b_2})+\boldsymbol{b_3}
\end{aligned}
\end{equation}
where $\boldsymbol{W_2} \in \mathbb{R}^{{d}\times {d}}$, $\boldsymbol{b_2} \in \mathbb{R}^{d}$, $\boldsymbol{W_3} \in \mathbb{R}^{\frac{d}{2} \times {d}}$, $\boldsymbol{b_3} \in \mathbb{R}^{\frac{d}{2}}$ are both trainable parameters. In the right tower, the compared embedding of the instance, namely $\mathbf{s}^s\in\mathbb{R}^{\frac{d}{2}}$, is obtained by the same operation in Eq. \ref{eq:project} where only prototype $\boldsymbol{p}$ is replaced by instance's representation $\boldsymbol{h}$.

\nop{
Specifically, hidden embeddings $\boldsymbol{h}_c$ from instances fed into the encoder layer together with the prototype $\boldsymbol{p}$, are inputted to projector:
\begin{equation}\label{eq:project}
\begin{aligned}
    \mathbf{s}=\boldsymbol{W_3} GELU(\boldsymbol{W_2}\left\{\boldsymbol{p},
    \boldsymbol{h}_c\right\}+\boldsymbol{b_2})+\boldsymbol{b_3},
\end{aligned}
\end{equation}
where $\left\{\boldsymbol{p},\boldsymbol{h}_c\right\}$ is $\boldsymbol{p}$ or $\boldsymbol{h}_c$, $\boldsymbol{p} \in \mathbb{R}^{d}$. $\boldsymbol{W_2} \in \mathbb{R}^{{d}\times {d}}$, $\boldsymbol{b_1} \in \mathbb{R}^{d}$, $\boldsymbol{W_3} \in \mathbb{R}^{\frac{d}{2} \times {d}}$, $\boldsymbol{b_1} \in \mathbb{R}^{\frac{d}{2}}$ are trainable parameters. 
}

Then, given a compared instance $i$, suppose its relation's compared embedding is $\mathbf{s}^r_{+}$, i.e., the only positive sample, we have our contrastive learning's InfoNCE loss \cite{oord2018representation} as
\begin{equation}\label{eq:contrast_loss}
\begin{aligned}
    \mathcal{L}_2=-\sum_{i=1}^{N}\log \frac{\exp \left(\mathbf{s}^s_{i} \cdot \mathbf{s}^r_{+} / \tau\right)}{\sum_{j=1}^{J} \exp \left(\mathbf{s}^s_{i} \cdot \mathbf{s}^r_{j}/ \tau\right)},
\end{aligned}
\end{equation}
where $\mathbf{s}^s_{i}$ is the compared embedding of instance $i$, $\boldsymbol{s}^r_j$ is the $j$-th relation's compared embedding, and $\tau$ is a temperature hyper-parameter. $N$ is the number of compared instances, and $J$ is the minimum between the number of all relations stored in the memory module (their typical instances are stored in fact) and batch size. %If instance $i$ does not belong to relation $j$, $(i, j)$ is regarded as a negative sample pair in the loss of Eq. \ref{eq:contrast_loss}. 
% 在这里我们将对比学习的训练建模为句子与其原型的对比：原型本身就是由特定关系r的所有句子信息得到的（原型本身就是处于类的中心位置），对于那些与这个原型属于相同类别的句子，我们认为其和原型具有相似性，否则则应该作为负样本。 具体来说对比网络由分类网络中的encoder和projector组成，在projector得到向量表示之后，再比较两个向量的相似度，计算损失函数。
%具体公式。。。loss表示。然后相似度嵌入s和同batch数据计算cos相似度。

\subsubsection{Two Training Processes of Contrastive Learning}
There are two training processes in our contrastive network, that follow the training process of the classification network introduced before. These two training processes both use the lnfoNCE loss in Eq. \ref{eq:contrast_loss}, to make the network parameters more fit to current task and all historical tasks, respectively.

In the first training process, the $N$ in Eq. \ref{eq:contrast_loss} is set to $N_k$. It indicates that the network parameters are fine-tuned by contrastive learning with respect to (w.r.t.) the instances in current task $T_k$, and thus enhance the relation extraction performance of $T_k$. However, it can not ensure the model fit to all tasks, because the model pays more attention to current task rather than the historical tasks during this training process. In other words, as we have explained in the example of Figure \ref{fig:res1}, the model tends to ensure the instances of different relations in $T_k$ distinguishable, but forgets to meanwhile keep the instances of different relations in all historical tasks also distinguishable. As a result, the model's catastrophic forgetting happens.

%In contrastive learning, the current task needs to be fitted first so that network parameters can be adjusted to increase the accuracy of the current task. In this case, the negative samples come from the samples in the current task that are not of the same class as the prototype. By performing the second training in this way, you can get a comparative learning model that fits well for the current task. But this is still not enough, during the above training process, the model did not learn how to distinguish between previous representations of relationships, re sulting in a serious catastrophic forgetting problem, which was demonstrated in our ablation experiments. So we need to learn about historical tasks, which leads to a third training.
% 对比学习首先需要对当前任务进行拟合，以便网络参数调整增加当前任务的准确率。此时负样本来源于当前任务中与原型不同类的样本。通过这样进行第二次训练，就可以得到一个对当前任务拟合较好的对比学习模型。但这样依然是不够的，在上述训练过程中，模型并没有学习到如何对以往的关系实例进行区分，因此会产生严重的灾难性遗忘问题，这一点在我们的消融实验中得到了验证。所以我们需要对历史任务进行学习，这带来了第三次的训练。

To alleviate the catastrophic forgetting in CRE, we need the second training process in the contrastive network. Specifically, we just set $N=L\times J$ in the loss of Eq. \ref{eq:contrast_loss}. It indicates that in this training process all typical instances stored in the memory module are compared, which represent the relations in all tasks. Accordingly, this training process can effectively prevent the model from catastrophic forgetting. 
%The techniques used in the third training are the same as those used in the second training, except for samples. Using the representation of L typical samples stored in memory, training can be performed. Similarly, we consider the sentences in memory that belong to the same class as the prototype as positive samples, and the sentences in the memory that are different from the prototype as negative samples, because memory has stored data information of historical tasks in the previous steps, so training in this step can effectively prevent the model from catastrophic forgetting. 

We have also tried to merge these two training processes. That is, both the stored typical instances and the instances of current task are used together as the compared instances. But due to the huge data gap, even if the Focal loss \cite{lin2017focal} was used for balance, there is still a serious catastrophic forgetting problem. Thus we finally adopted the strategy of three separate training processes, i.e., the training in the classification network, followed by the two training process in the contrastive network. The previous work \cite{han2020continual,cui2021refining} also called this strategy as memory reconsolidation.
%第三次训练所使用各项技术与第二次训练相同，除了采样的样本。使用在memory中存储下来的L个典型样本表示，就可以进行训练。类似的，我们将memory中与原型属于相同类的句子认为是正样本，将memory中与原型不同的类别句子认为是负样本，由于memory已经在前述步骤中存入了历史任务的数据信息，所以在这一步的训练可以有效地防止模型灾难性遗忘。我们也尝试了将第二次和第三次训练合并，即训练数据既包含历史数据，也包含当前任务的新数据，但由于数据量差距悬殊，哪怕使用了Focal loss进行平衡，在这种情况下依旧会发生严重的灾难性遗忘问题，因此我们使用了三次训练的方法，以往的工作\cite也把这种方法称为Memory Reconsolidation。


\subsection{Prediction}
% 在一个新的句子到来的时候，我们只需要衡量句子与memory中通过encoder-middle layer及平均操作计算所得到的原型表示的相似性即可，也就是说我们只需要衡量句子与哪个原型最相似，就可以把句子判断为这个类别。
Besides model training, the contrastive network is also used to achieve relation prediction (classification) for the test samples. Specifically, when a new instance arrives, we only need to measure its similarity to all stored relation prototypes, which is computed as the cosine distance between the instance's representation and the compared prototype. Then, we choose the relation (prototype) with the highest similarity as the prediction result. As we emphasized in Section 1, such contrasting-based mechanism ensures our framework's capability of class-incremental learning in CRE.

\begin{algorithm}[!htb]
\small
\caption{Training procedure for $T_k$}\label{alg1}
\LinesNumbered
\KwIn{$D_k$, $R_k$, $\tilde{R}_{k-1}$, $\tilde{M}_{k-1}$}
\KwOut{ $\tilde{M}_{k}$} % $\tilde{R}_{k}$,sentence encoder \emph{\textbf{E}}, linear classifier \emph{\textbf{C}},  memory network \emph{\textbf{M}}
%\begin{algorithmic}[1]
%   $\mathcal{P}_k \gets \emptyset$\;
  \For{$i$ = 1 to epochs1}
{
     train classification model according to $\mathcal{L}_1$ on $D_k$\;
}
    $\tilde{R}_{k}=\tilde{R}_{k-1} \cup R_k$
  \For{each $r \in R_k$}
  {
  	get data $d_r$ from $D_k$\;
  	get $\boldsymbol{h}$ by Eq.\ref{eq:dropout}\;
  	apply K-means to $\boldsymbol{h}$ and select $L$ samples to memory $M_{k}$\;
 }
 \For{each $r \in \tilde{R}_{k}$}
 {
    get $\boldsymbol{h}$ by Eq.\ref{eq:dropout}\;
    get prototype $\boldsymbol{p}$ by average $h$ of relation $r$\;
 }
    generate contrastive training data $C_k$ by sampling from $D_k$\;
   \For{$i$ = 1 to epochs2}
{
     train contrastive model according to $\mathcal{L}_2$ on $C_k$ and $\boldsymbol{p}$\;
}
    generate contrastive training data $\tilde{C_k}$ by sampling from $\tilde{M}_{k}$\;
\For{$i$ = 1 to epochs3}
{
     train contrastive model according to $\mathcal{L}_2$ on $\tilde{C_k}$ and $\boldsymbol{p}$\;
}
\end{algorithm}




